First principles studies of the electronic and structural properties of the rutile VO$_{2}$(110) surface and its oxygen-rich terminations

We present a Density Functional Theory (DFT) study of the structural and electronic properties of bare rutile VO$_{2}$(110) surfaces and its oxygen-rich terminations. We discuss the performance of various DFT functionals, including PBE, PBE+U (U = 2 eV), SCAN and SCAN+rVV functionals with non-magnetic and ferromagnetic spin ordering. We predict the presence of a ring-like termination that is electronically and structurally related to a V$_{2}$O$_{5}$(001) monolayer and shows a higher stability than pure oxygen adsorption phases. Despite the fact that the calculated phase stabilities depend on the chosen functional, our results show that employing the spin-polarized SCAN functional offers a good compromise yielding both a reasonable description of the structural and electronic properties of the rutile VO$_{2}$ bulk phase and the enthalpy of formation for different stages of vanadium oxidation.

==> abstract.tex <==
\begin{abstract}

\end{abstract}


